Tailor: Generating and Perturbing Text with Semantic Controls

Controlled text perturbation is useful for evaluating and improving model generalizability. However, current techniques rely on training a model for every target perturbation, which is expensive and hard to generalize. We present Tailor, a semantically-controlled text generation system. Tailor builds on a pretrained seq2seq model and produces textual outputs conditioned on control codes derived from semantic representations. We craft a set of operations to modify the control codes, which in turn steer generation towards targeted attributes. These operations can be further composed into higher-level ones, allowing for flexible perturbation strategies. We demonstrate the effectiveness of these perturbations in multiple applications. First, we use Tailor to automatically create high-quality contrast sets for four distinct natural language processing (NLP) tasks. These contrast sets contain fewer spurious artifacts and are complementary to manually annotated ones in their lexical diversity. Second, we show that Tailor perturbations can improve model generalization through data augmentation. Perturbing just 2% of training data leads to a 5.8-point gain on an NLI challenge set measuring reliance on syntactic heuristics.

==> _outline.tex <==
Intro 

Motivation: Closely related examples are useful for various applications. Existing methods to create them are limited (rely on human annotations or crafted heuristics). Recent work has shown that creating such examples with generators can support various applications while greatly saving human efforts. However, these generators usually only follow sparse and ad-hoc signals, which may have limited coverage (Polyjuice only has a preset control codes), introduce some bias (Polyjuice trained on paired data), or under-specify the desired changes (MiCE instructs positive→negative which may be translated to multiple possible changes.)

We propose a general-purpose generator for creating closely related examples that takes more formal and finer-grained controls. At training time, it takes both structured labels and content keywords as control signals. At generation time, the combinations of label and keyword helps to get interesting meaningful data recombinations. By varying the sampling strategy of data recombination, the generator can power different downstream tasks (this is a bit like Polyjuice's argument on task-agnostic counterfactual generation model + task-dependent counterfactual selection method.) We show that our generator can be used to create contrastively edited inputs for a variety of tasks.

Contributions
1. We design a generator for producing closely related examples. Key designs are: 
- Use structured labels as primary controls, which effectively adopt well-established, high-dimensional linguistic features, making the control signal more flexible (compared to the small set of ad-hoc lists in Polyjuice) and nuanced (compared to low level classification labels in MiCE).
- Use content keywords to allow for data recombination, which gives the potential of targeting at rare patterns in data collection, rather than just randomly querying the generator (the latter may even induce some biases, e.g., if using models trained on paired data like Polyjuice)
- The format of head control codes + multiple blanks disentangle the "where" (placement) and "what" (content) of the perturbation.
- Use unlikelihood training to enhance controllability without requiring paired data (as in Polyjuice)
- Use perplexity filtering [and cycle consistency or some IE heuristic / some additional ranking techniques] to enhance validity while maintaining diversity




* Method
---
** Model

We design a generator for producing closely related examples. Key designs are:
- Use structured labels as primary controls, which effectively adopt well-established, high-dimensional linguistic features, making the control signal more flexible (compared to the small set of ad-hoc lists in Polyjuice) and nuanced (compared to low level classification labels in MiCE).

- Use content keywords to allow for data recombination, which gives the potential of targeting at rare patterns in data collection, rather than just randomly querying the generator (the latter may even induce some biases, e.g., if using models trained on paired data like Polyjuice)
The format of head control codes + multiple blanks disentangle the "where" (placement) and "what" (content) of the perturbation.

- Use unlikelihood training to enhance controllability without requiring paired data (as in Polyjuice)
Use perplexity filtering [and cycle consistency or some IE heuristic / some additional ranking techniques] to enhance validity while maintaining diversity


** Perturbation strategies
- Design rationale + actual strategies (and their mapping to the SRL labels) + [appendix on how they are used in different challenge sets]

* Evaluation
*** Intrinsic evaluation
- Metrics:
    - Fluency of generated sentences
    - Minimality of edits (for ex: if we are only changing a temporal modifier, the rest of the sentence should remain unchanged)
    - Proportion of tags followed (as measured by SRL predictor, cycle consistency; + manual)
    - Proportion of keywords followed
- Ablation studies measuring the impact of unlikelihood training on tag following/keyword following


* Applications
** Data augmentation
- NLI
- Matres
- [improve on contrast sets]

** Case studies on creating contrast sets for QA, dependency parsing


* Related work
** Doing counterfactual/perturbation-based analysis (challenge/contrast set)
- Lit, challenge set

** Models doing counterfactual perturbations (can be part of the above)
- Polyjuice, MiCE
- Data recombination
- Automatic Generation of Contrast Sets from Scene Graphs: Probing the Compositional Consistency of GQA



==> sections/__backup_generator.tex <==
\section{\sysname: Designing a Controllable Generator}
\label{sec:generator-design}
% }\matt{+1.  You also need some kind of intro text here that gives a high-level outline of the method, which might look something like, ``In this section we describe how we use SRL labels to create control codes for a generative model, how use those control codes inside of prompts to generate text, and how we train the generative model.''}

In this section, we provide an overview of \sysname, a generator designed to be controllable at various levels of abstraction. First (\sect{ssec:control-codes}), we motivate and outline our \textbf{control codes}, which build on Semantic Role Labeling (SRL) labels and specify the desired form of the generated text. Next (\sect{ssec:prompts}), we describe how we combine control codes within \textbf{prompts}, or inputs to the \sysname generator, to allow for varying degrees of control over the generated text. Finally (\sect{ssec:training}), we describe how we use \textbf{unlikelihood training} to train our generator to follow the specified control codes.

\input{tables/controls}

\begin{comment}
\begin{figure}[t]
\centering
\includegraphics[trim={0 8cm 30cm 0cm}, clip, width=1\columnwidth]{figures/prompt_design_2}
\vspace{-15pt}
\caption{
The design of the prompt. 
\wts{See the description in the full text for now. Not sure if this is too compact...}
}
\vspace{-10pt}
\label{fig:prompt_design}
\end{figure}
\end{comment}

\subsection{Control Codes}
\label{ssec:control-codes}
% We design our generator in order to have fine-grained control over generated content. 


\wts{
We should probably add some more motivation on why we choose to abstract the sentences in this way. Would it make sense if some part of 3.1 is the motivation of this?

2.1 - Information encoded in the control header
\begin{compactenum}
\item reviewing existing perturbations, it is most essential that we can control the content of the generated/perturbed sentences (e.g. sentence expansion/abstraction, recombination etc.)
\item So, our goal is to design a generator with fine-grained control on sentence semantics.
\item To make it generalizable, we choose to do a combination of SRL label + content keyword, with SRL controlling the shallow, thematic role (agent, patient), whereas content key controls the actual verb and arguments -- which may need to be very specific or not specified at all depending on different applications (example?). 
\item alternatives: why SRL over AMR and dep parsing (maybe too fine-grained? Hard to decide what to encode and what not to, e.g. marks? https://arxiv.org/pdf/2010.11170.pdf)
\item Further, we add controls on the predicate verb, as well as the fill-in-the-blank structure to achieve additional syntactic control on where a semantic role should be inserted.
\end{compactenum}

2.2 - Constructing the prompt
\begin{compactenum}
\item our goal is to encode all the information mention in 2.1 in an abstract way, and finetune the model to reconstruct the full sentence.
\item readable label
\item extra blank
\item subset of roles
\end{compactenum}

2.3 - training
\begin{compactenum}
\item data
\item unlikelihood training
\end{compactenum}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Semantic Role Labeling (SRL) is the task of determining the predicate-argument structure of a sentence. The goal of SRL is to identify ``who did what to whom'' and involves analyzing a sentence's \textit{predicates}, usually verbs representing events (i.e. ``what'' happened), and predicate \textit{arguments}, which specify abstract, thematic roles of the predicate (i.e. ``who,'' ``to whom'', ``where,'' ``how,'' etc.) ~\citep{ palmer-etal-2005-proposition}. 
A predicate takes \textit{core} arguments, which specify the key thematic roles in the predicate, as well as \textit{adjunct} arguments, which are modifiers providing additional information. For example, in Figure \ref{fig:teaser}, the predicate ``comforted'' has {core} arguments ``the doctor'' and ``the athlete,'' as well as adjunct argument ``In the operation room.'' Because SRL labels reflect well-established high-dimensional linguistic features, key SRL labels are generalizable across languages \citep{hajic-etal-2009-conll}.
% \hao{a quick dedicated review of SRL would be great before diving in. I think this is what most NLP folks enjoy seeing. And this could help justifying using SRL, and make the transition to later sections smooth.} 
% \matt{Also, related to Hao's point, is there a universal SRL tag set, like there is for universal dependencies? Can we say anything about multi-linguality of this kind of generation model? Any discussion of that would go in the background SRL section.}

We adopt SRL labels as primary control codes for \sysname, allowing for control over the semantic content of generated text. As shown in Table \ref{tab:controls}, we map original SRL labels to human-readable labels (i.e.\, \optag{ARG0} $\rightarrow$ \optag{AGENT}) in order to leverage latent knowledge learned by pretrained models about the meaning of role labels \citep{paolini2021structured}.\footnote{We map \optag{ARG0} $\rightarrow$ \optag{AGENT} and \optag{ARG1} $\rightarrow$ \optag{PATIENT}. For other numbered arguments, we create human-readable labels by using argument functions \alexis{Is that what the f attribute is?} included in PropBank frame for the given predicate \citep{palmer-etal-2005-proposition}.}

In addition to these primary controls, fine-grained controls modulate the syntactic form of text generated with \sysname. These 
% secondary controls 
are: \textit{voice, tense, lemma} for verbs and \textit{keyword content, keyword specificity} for semantic roles. For each semantic role, the \textit{keyword content} and \textit{keyword specificity} controls allow us to vary to what extent we are recombining existing text vs. generating new text.
% \hao{this sent doesn't parse for me}
% and recombine of varying amounts of existing text. 
For instance, to generate a span like ``under the dim light in the operation room,'' the following combinations of ({keyword content}, {keyword specificity}) could be used, listed in decreasing likelihood of generating the exact target span: (\optag{complete}, \textit{under the dim light in the operation room}), (\optag{partial}, \textit{dim light in the operation room}), (\optag{partial}, \textit{operation room}), (\optag{sparse}, \textit{under}), (None, \optag{*}).

\subsection{Prompts}
\label{ssec:prompts}
\input{tables/example_prompts}
% At training time, given a sentence and a corresponding SRL structure on it, we extract various information per structural block.
% For all blocks, we extract keywords that can either be \emph{complete} (\ie the entire phrase, like ``the doctor''), \emph{partial} (\eg noun chunks or random subtrees that covers a large portion of the phrase, like ``athlete''), or \emph{sparse} (\eg connecting prepositions like ``in'' in (B)).
% In addition, for the predicate verb (\tlabel{VERB}), we also annotate its voice (active/passive) and tense (past/future/present). 
% \matt{Start with a declarative description: ``A prompt is a \dots''.  Then ``Prompts can be obtained in many different ways; for perturbation-based uses of \sysname, which we focus on in this paper, a sentence needs to be first \dots'' (whenever I give text like this it's just intended to be a starting point for something better, not necessarily polished text you should use in the paper)}

A prompt is an input to a generator model that specifies what form the generated text should take. Prompts can take a variety of forms, including sentence prefixes \citep{Gehman2020RealToxicityPromptsEN} or cloze-style (i.e.\, ``fill in the blank'') phrases \citep{Petroni2019LanguageMA,Schick2021ExploitingCF}. 
% We design prompts to the \sysname generator to allow for varying degrees of control over generation.
In our case, \sysname prompts encode control codes to follow, target text to include, and context to preserve in a generation. 
In the rest of this section, we describe how our prompt design allows for flexible, controllable generation and facilitates perturbation-based uses of \sysname, which we focus on in this paper.

A \sysname prompt consists of a \textit{header} and \textit{context}. As shown in Table \ref{tab:example-prompts}, the header is bracketed and contains our control codes (\sect{ssec:control-codes})--SRL labels and fine-grained controls such as target text to include. The context consists of natural language and \textit{blank} tokens: The text in the context represents text that should be preserved, and blank tokens specify where any new text following controls in the headers should be generated.
% relative to the original context. 

% The generator is designed to generate text in the blank locations that follows control codes in the header while preserving any original text in the context.

% For instance, for the sentence shown in Figure \ref{fig:prompt_design}, i.e.\, \textit{In the operation room, the doctor comforted the athlete}, one prompt could be: [\theaderVerb{active}{past}{comfort} | \theader{AGENT}{complete}{the doctor} | \theader{PATIENT}{partial}{athlete} | \theader{LOCATIVE}{partial}{in}] \tblank{0} \tblank{1} \tblank{2} \tblank{3} \tblank{4}. 
% Given such a prompt, the generator outputs the original sentence augmented with primary SRL-derived control codes.
% , as shown in Figure \ref{fig:prompt_design}. 
% As for the output format, we augment the original natural sentence with the SRL labels, so the model learns the mapping between the header control in the input and the generated output, rather than randomly involving doctor and athlete as patient and agent respectively.

Beyond flexible controls, several prompt design choices allow for varying degrees of control over generation. Firstly, because we lack information about the optimal ordering of SRL arguments at generation time, we encode SRL controls without information about the positions of their corresponding spans in the target sentence.
% \hao{I would start by saying that at generation time one does not have access to the optimal ordering, that's why} 
% we encode controls for semantic roles without information about the positions of their corresponding spans in the target sentence.
Excluding positional information from the header allows the model to flexibly recombine the given roles in the most fluent way.
% at generation time.
For instance, we do not order controls by their relative orders in target sentences, but rather begin every prompt header with the verb (\optag{VERB}), then core arguments (\optag{AGENT}, \optag{PATIENT}), and randomly ordered noncore arguments (\optag{LOCATIVE}, \optag{TEMPORAL}, etc.); this input-independent ordering discourages the generator from learning to generate text solely in the order in which the arguments appear in the header. 

Secondly, our prompts can include varying degrees of blanking. Our generator can take prompts that (a) only blank a subset of SRL roles (i.e.\, example B in Table \ref{tab:controls}), and (b) insert extra empty blanks (i.e.\, example C).
% , and (c) `overblank' context--i.e.\, blank punctuation and other tokens that do not constitute SRL roles for a given verb. 
(a) allows us to minimally perturb original sentences at generation time; for instance, we may only want to change the tense of a verb, in which case we would want to only blank the verb. (b) encourages invariance to the exact location of blanks such that at generation time, text can be recombined fluently when exact desired locations of such data is unknown. 
% Similarly, (c) allows for minor edits to context when necessary to encourage grammaticality of perturbed text. 
Together, these design choices help modulate the tradeoff between strict control, which facilitates minimal perturbations, and flexibility of generation, which allows for natural-sounding text. In \sect{sec:evaluation}, we evaluate the impact of these choices on the controllability of our resulting generator.
% [\theaderVerb{active}{past}{comfort} | \theader{AGENT}{complete}{the doctor} | \theader{PATIENT}{partial}{athlete}] In the operation room, \tblank{0} \tblank{1} \tblank{2} \tblank{3}. 
For more information about the specifics of prompt formats, see \sect{sec:prompt-format}.
% \matt{I haven't finished reading the paper yet, but this section reads to me like a promise to evaluate some of these choices. Do you have ablations that explore the actual impact of these things?}
% \matt{Also, I think this section could use some restructuring. Might be easier to talk this through in person.}

% \hao{suggest introducing what the generator is supposed to do (which is yet clear) before talking about training details. I would put this upfront, maybe at the start of this section.}
\subsection{Training}
\label{ssec:training}
We use the OntoNotes 5.0 data \citep{pradhan-etal-2013-towards} as training data and \textsc{T5-base} \citep{2020t5} as our generator. We create prompts using gold SRL annotations in OntoNotes 5.0 and train our generator to output original sentences augmented with primary SRL-derived control codes, as shown in Table \ref{tab:example-prompts}. In order to train our generator to be sensitive to the different prompt formats described above, for each original prompt, we randomly sample: the number of SRL arguments to blank, the number of extra empty blanks, 
% whether to overblank the context \alexis{confirm}, 
and keyword content/keyword specificity for each role. 

A key issue in training our generator to be controllable is that standard likelihood training is insufficient for encouraging control code following, as there may exist signal beyond the control codes for the form that a generation should take. Consider the prompt [\theaderVerb{{active}}{{past}}{comfort} | \theader{{TEMPORAL}}{{partial}}{in}] \tblank{0}, the doctor \tblank{1} \tblank{2} the athlete. Given the context of ``the doctor'' and keyword ``in,'' for the span [\theader{{TEMPORAL}}{{partial}}{in}], a generator trained with standard likelihood training may output text pertaining to where a medical appointment may take place, such as ``in the hospital,'' if the training data contains a bias towards including location phrases for keyword ``in'' and medicine-related phrases when a context contains ``doctor.''

In order to enforce reliance on controls like \optag{TEMPORAL} rather than other signals, we use \textbf{unlikelihood training} \citep{Welleck2020Neural} to penalize our generator for generating text that does not follow controls. We create `negative' samples by randomly perturbing the control codes in our header. See the last row in Table \ref{tab:example-prompts} for an example. Intuitively, we penalize the generator for generating a sequence that does not follow the control codes---i.e.\, a sequence with a past, active verb (which does not follow verb controls \optag{passive} and \optag{future}) and a span specifying the location of the comforting (rather than when it happened, such as \textit{In 2010}, given primary control \optag{TEMPORAL}). We create three  negative samples per prompt, which randomly perturb: 1) verb voice/tense, and primary controls for SRL arguments, 2) keyword contents, and 3) keyword specificities. See \sect{ssec:training-prompts} for details.

% In \sect{sec:evaluation}, we explore the efficacy of unlikelihood training through an ablation study.\matt{Having this as a contribution is already an implicit promise to do an ablation. No need to put this here.}

% flip out certain metadata (the redden parts in the figure) to create negative samples.
% With random combinations of these metadata, we get multiple input prompts per sentence.
% Note that not all structures have to be blocked: In Figure~\ref{fig:prompt_design}C2, it is possible to leave the locative modifier out, and only create headers and blanks for the core arguments and the verb.

==> sections/__backup_introduction.tex <==
\section{Introduction}
\label{sec:introduction}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The high dimensional, discrete nature of text data inevitably leads to sparsity-driven biases and distributional gaps in most---if not all---existing NLP datasets~\cite{gardner2020evaluating}.
As a result, NLP models trained on such datasets learn to rely on spurious features, rather than 
% the true, complex decision boundary.
learning true, complex decision boundaries.
One promising way to overcome data sparsity is by constructing new examples that are closely related to those already in a dataset. Prior work has shown that perturbations on existing data points (as in Figure~\ref{fig:teaser}) can help mitigate dataset biases~\cite{gardner2021competency}, explain model behaviors~\cite{ross2020explaining}, and improve model generalization~\cite{teney2020learning}.


\begin{figure}[t]
\centering
\includegraphics[trim={0 9cm 30cm 0cm}, clip, width=1\columnwidth]{figures/teaser}
\vspace{-15pt}
\caption{
A showcase of compositional perturbation using \sysname.
Given (A) an original sentence and its SRL structure, we abstract each span into a structured header that contain its semantic roles and keywords, and specify the desired perturbations by modifying each control code (change the role \swap{\texttt{LOCATIVE}}{\texttt{TEMPORAL}} in (B), verb tense \swap{past}{present}, and patient keyword specificity \swap{complete}{sparse}).
With the \emph{perturbed control codes} prepended to the input prompt (C), \sysname generates a new sentence that follows all the perturbation controls, recombininng data spans that are not explicitly in the training data.}
\vspace{-10pt}
\label{fig:teaser}
\end{figure}

Despite their effectiveness, creating such close examples is challenging.
Most methods rely on human annotations~\cite{kaushik2019learning,gardner2020evaluating} that are costly to scale and liable to systematic omissions, or strictly crafted heuristic rules that have limited generality~\cite{li-etal-2020-linguistically}.
While automated generation can effectively save human effort, prior works 
% Existing methods for automatic generation of perturbations
frequently specify generators for a limited set of perturbation strategies. 
They 
% would 
first identify certain useful perturbations, 
% (\eg \emph{negation} like \swap{great}{not great}~\cite{polyjuice:acl21}, or \emph{past tense} like \swap{run}{ran}~\cite{akyurek2020learning}), 
collect paired data points that demonstrate such strategies, and train with such data pairs to directly embed the strategies into the generator.
As a result, extending the generator's coverage is expensive --- adding a new perturbation requires not only re-training, but also extensive annotations of training pairs, which do not naturally exist for most perturbations.

In this work, we seek to broaden the coverage of perturbation strategies with \sysname, by disentangling perturbation strategies from generator training.
%In this work, we overcome this limitation with \sysname, a flexible, controllable generator that can implement a \textit{variety} of perturbations by building on linguistic properties of text, rather than particular perturbation strategies. 
\sysname contains two parts: 
First, we build a \sysname generator, a flexible, controllable generator that generates full sentences from desired linguistic properties.
% , which builds on T5~\cite{2020t5}, 
%to be controllable through carefully designed inputs and training mechanisms. 
Inspired by AMR (Abstract Meaning Representations)-to-Text generation~\cite{mager2020gpt}, our \textbf{prompts} (\sect{ssec:prompts}) represent desired outputs with a series of abstract, structured control codes, as shown in Figure~\ref{fig:teaser}.
% (\eg \optag{LOCATIVE+sparse:in} in Figure~\ref{fig:teaser}).
Each code is built on Semantic Role Labels (SRL) and specifies the semantics of a span in the targeted sentence, through ``who did what to whom''~\cite{palmer-etal-2005-proposition}. 
The high-dimensional SRL labels make \sysname controllable at a more fine-grained level than existing generators and style transfer methods~\cite{ross2020explaining, madaan2020generate}, which rely on sparse
% (two- or three- dimension classification)
labels that under-specify desired changes. 
 We also use \textbf{unlikelihood training} (\sect{ssec:training})~\cite{Welleck2020Neural} to encourage
%  \matt{encourage? ``enforce'' sounds like a constraint}
 control code following. In \sect{sec:evaluation}, we evaluate the effect of these choices on the flexibility and controllability of \sysname.

% Inspired by AMR (Abstract Meaning Representations)-to-Text generation~\cite{mager2020gpt}, we represent the desired output with a series of abstract, structured headers in the input (\eg \optag{LOCATIVE+sparse:in} in Figure~\ref{fig:teaser}).
% Each header includes Semantic Role Labels (SRL) and the desired content keywords, specifying `who did what to whom'', ``when'', and ``where.''~\cite{palmer-etal-2005-proposition}.
% Based on these headers, we finetune T5~\cite{2020t5} with carefully designed input prompts and training mechanism such that, given the control headers and the blanking placements, \sysname recover the full sentence in a way that follows the predicate-argument structure \emph{and} the content constraints.
% For example, through unlikelihood training~\cite{Welleck2020Neural}, we discourage generation of outputs that do not match the given control; through inserting additional blanks, \sysname learns to match blank positions with the corresponding arguments, and can generate grammatical sentences by re-ordering the arguments.

% Then, we apply \sysname for perturbations, by editing the input abstract headers.
% With the labels being high-dimensional, \sysname accepts finer-grained controls compared to existing generators and style transfer methods~\cite{ross2020explaining, madaan2020generate} that rely on sparse (two- or three- dimension classification) labels, as the latter tend to under specify the desired change, \eg merging \swap{great}{not great} and \swap{great}{bad} into a single \emph{}{Positive sentence to Negative sentence} control signal.
% Therefore, we can easily identify a variety of primitive operations that can modify the headers for syntactic rewrites (\eg \optag{CHANGE\_TENSE} in Figure~\ref{fig:teaser}), sentence expansion and abstraction (\eg \optag{CHANGE\_SPEC} which asks \sysname to extend ``the athlete''), as well as data recombination (\eg \optag{CHANGE\_TAG} that retrieves temporal information from \sysname).
% Through compositions of these primitives, \sysname enables effective defining new perturbation strategies during generation time, and hence make the perturbation coverage more flexible.

% \hao{haven't finished reading, but 
% it seems the following can be better structured:
% we showcase two applications of \sysname (we can hint more),
% (1) create challenge set with little human efforts;
% (2) improve the robustness and generalization using data augmentation. 
% the first one might be a bit tricky since we only used \sysname to 
% replicate existing challenge set, but never actually created a new one.
% }

Then, on top of the generator, we identify and implement a list of primary perturbation strategies as operations on input prompts (\sect{sec:perturbations}).
By composing these primitive operations, we can easily build complex perturbation strategies, without the need for repeating training or creating paired debiasing datasets for each perturbation we wish to implement. 
For example, in Figure~\ref{fig:teaser}, while it would nontrivial to directly train a generator to transform sentence A to D, we can achieve the transformation through a series of syntactic rewriting (changing the verb tense to present), sentence expansion (extending ``the athelete''), data recombination (\ie sourcing \optag{TEMPORAL} constraint).

We illustrate how \sysname can be used to implement more complex perturbations useful for three distinct applications: 
1) constructing \textbf{contrast sets} (\sect{sec:contrast_set}): We use \sysname to replicate existing challenge sets on four diverse tasks, with much less manual annotation effort. Our analysis suggests that these contrast sets result in valid instances, retain lexical diversity, and reduce dataset bias. 
2) improving robustness through \textbf{data augmentation} (\sect{sec:data_augment}): We show that augmenting training data with \sysname perturbations improves the robustness of Natural Language Inference (NLI) models to inference heuristics, as measured by the HANS evaluation set~\cite{mccoy2019right}. 
% \textbf{2) Minimizing human efforts in contrast set construction}
3) improving compositionality in \textbf{fine-grained style transfer} (\sect{sec:style_transfer}): \sysname achieves impressive zero-shot performance on fine-grained and compositional transfers in the \textsc{StylePTB} benchmark \citep{Lyu2021StylePTBAC}, even outperforming models trained on the dataset.

% We show that \sysname can help mitigate the data sparsity issues in various downstream tasks.
% In Natural Language Inference (NLI), we replicate perturbation strategies presented in HANS~\cite{mccoy2019right}, and use them to perturb the actual SNLI~\cite{bowman2015large} instances (instead of the templated data in HANS).
% The produced data, when automatically labeled, significantly improves NLI model generalization, on both HANS and other NLI challenge sets.
% In addition, \sysname helps replicate exisiting challenge sets on four diverse tasks, with much less manual annotation effort.
% We opensource \sysname at \opensourceurl.


==> sections/__backup_introduction_2.tex <==
\section{Introduction}
\label{sec:introduction}


\begin{figure}[t]
\centering
\includegraphics[trim={0 9cm 30cm 0cm}, clip, width=1\columnwidth]{figures/teaser}
\vspace{-15pt}
\caption{
A showcase of compositional perturbation using \sysname.
Given (A) an original sentence and its SRL structure, we abstract each span into a structured header that contain its semantic roles and keywords, and specify the desired perturbations by modifying each control code (change the role \swap{\texttt{LOCATIVE}}{\texttt{TEMPORAL}} in (B), verb tense \swap{past}{present}, and patient keyword specificity \swap{complete}{sparse}).
With the \emph{perturbed control codes} prepended to the input prompt (C), \sysname generates a new sentence that follows all the perturbation controls, recombininng data spans that are not explicitly in the training data.}
\vspace{-10pt}
\label{fig:teaser}
\end{figure}

Recently, controlled text generation has been the backbone for various tasks that involve text perturbation.
Given an original sentence, a controlled generator would modify its spans related to certain perturbation targets, while leaving the other parts intact (as in Figure~\ref{fig:teaser}); 
they have been shown to successfully modify sentence styles~\cite{reid2021lewis}, mitigate dataset biases~\cite{gardner2021competency}, explain model behaviors~\cite{ross2020explaining}, and improve model generalization~\cite{teney2020learning}.

Despite the wild success, prior work frequently trains the generators with sparse and application-specific control codes (\eg style transfer usually uses sentiment labels \emph{positive} and \emph{negative}).
Such design inevitably limits models' generalizabability to perturbation targets that have yet to be defined, as adding a new perturbation requires not only re-training, but also extensive annotations of source-target sentence training pairs.
%, which do not naturally exist in most cases.
More importantly, existing control codes tend to overly condense various possible perturbations that reflect different linguistic phenomena.
\eg merging \swap{great}{not great} and \swap{great}{bad} into a single \emph{positive}\arrow\emph{negative}~\cite{ross2020explaining, madaan2020generate}.
The under-specification becomes the bottleneck for finer-grained perturbations, which are usually important for generating datasets that evaluate and improve model's natural language understanding~\cite{kaushik2019learning, polyjuice:acl21}.


% With the labels being high-dimensional, \sysname accepts finer-grained controls compared to existing generators and style transfer methods~\cite{ross2020explaining, madaan2020generate} that rely on sparse (two- or three- dimension classification) labels, as the latter tend to under specify the desired change, 

In this work, we seek to ground our perturbations on well-established linguistic features, so to achieve fine-grained controls on where to perturb and how --- which also broaden the coverage of perturbation targets.
\wts{Let's maybe rename perturbation strategies in sec 5-7 into targets?}
%In this work, we overcome this limitation with \sysname, a flexible, controllable generator that can implement a \textit{variety} of perturbations by building on linguistic properties of text, rather than particular perturbation strategies. 
\sysname contains two parts: 
First, we build a \sysname generator, a flexible, controllable generator that generates full sentences from desired linguistic properties.
% , which builds on T5~\cite{2020t5}, 
%to be controllable through carefully designed inputs and training mechanisms. 
Inspired by AMR (Abstract Meaning Representations)-to-Text generation~\cite{mager2020gpt}, our \textbf{prompts} (\sect{ssec:prompts}) represent desired outputs with a series of abstract, structured control codes, as shown in Figure~\ref{fig:teaser}.
% (\eg \optag{LOCATIVE+sparse:in} in Figure~\ref{fig:teaser}).
Each code is built on Semantic Role Labels (SRL) and specifies the semantics of a span in the targeted sentence, through ``who did what to whom''~\cite{palmer-etal-2005-proposition}. 
The high-dimensional SRL labels lends \sysname the ability to perform fine-grained controls on each individual arguemnts within a sentence (\eg one can just change the patient span in Figure~\ref{fig:teaser}).
We also use \textbf{unlikelihood training} (\sect{ssec:training})~\cite{Welleck2020Neural} to encourage
%  \matt{encourage? ``enforce'' sounds like a constraint}
 control code following. In \sect{sec:evaluation}, we evaluate the effect of these choices on the flexibility and controllability of \sysname.

% Inspired by AMR (Abstract Meaning Representations)-to-Text generation~\cite{mager2020gpt}, we represent the desired output with a series of abstract, structured headers in the input (\eg \optag{LOCATIVE+sparse:in} in Figure~\ref{fig:teaser}).
% Each header includes Semantic Role Labels (SRL) and the desired content keywords, specifying `who did what to whom'', ``when'', and ``where.''~\cite{palmer-etal-2005-proposition}.
% Based on these headers, we finetune T5~\cite{2020t5} with carefully designed input prompts and training mechanism such that, given the control headers and the blanking placements, \sysname recover the full sentence in a way that follows the predicate-argument structure \emph{and} the content constraints.
% For example, through unlikelihood training~\cite{Welleck2020Neural}, we discourage generation of outputs that do not match the given control; through inserting additional blanks, \sysname learns to match blank positions with the corresponding arguments, and can generate grammatical sentences by re-ordering the arguments.

% Then, we apply \sysname for perturbations, by editing the input abstract headers.
% With the labels being high-dimensional, \sysname accepts finer-grained controls compared to existing generators and style transfer methods~\cite{ross2020explaining, madaan2020generate} that rely on sparse (two- or three- dimension classification) labels, as the latter tend to under specify the desired change, \eg merging \swap{great}{not great} and \swap{great}{bad} into a single \emph{}{Positive sentence to Negative sentence} control signal.
% Therefore, we can easily identify a variety of primitive operations that can modify the headers for syntactic rewrites (\eg \optag{CHANGE\_TENSE} in Figure~\ref{fig:teaser}), sentence expansion and abstraction (\eg \optag{CHANGE\_SPEC} which asks \sysname to extend ``the athlete''), as well as data recombination (\eg \optag{CHANGE\_TAG} that retrieves temporal information from \sysname).
% Through compositions of these primitives, \sysname enables effective defining new perturbation strategies during generation time, and hence make the perturbation coverage more flexible.

% \hao{haven't finished reading, but 
% it seems the following can be better structured:
% we showcase two applications of \sysname (we can hint more),
% (1) create challenge set with little human efforts;
% (2) improve the robustness and generalization using data augmentation. 
% the first one might be a bit tricky since we only used \sysname to 
% replicate existing challenge set, but never actually created a new one.
% }

Then, on top of the generator, we identify and implement a list of primary perturbation strategies as operations on input prompts (\sect{sec:perturbations}).
By composing these primitive operations, we can easily build complex perturbation strategies, without the need for repeated annotation or training. %or creating paired debiasing datasets for each perturbation we wish to implement. 
For example, in Figure~\ref{fig:teaser}, while it would nontrivial to directly train a generator to transform sentence A to D, we can achieve the transformation through a series of syntactic rewriting (changing the verb tense to present), sentence expansion (extending ``the athelete''), data recombination (\ie sourcing \optag{TEMPORAL} constraint).

We illustrate how \sysname can be used to implement more complex perturbations useful for three distinct applications: 
1) constructing \textbf{contrast sets} (\sect{sec:contrast_set}): We use \sysname to replicate existing challenge sets on four diverse tasks, with much less manual annotation effort. Our analysis suggests that these contrast sets result in valid instances, retain lexical diversity, and reduce dataset bias. 
2) improving robustness through \textbf{data augmentation} (\sect{sec:data_augment}): We show that augmenting training data with \sysname perturbations improves the robustness of Natural Language Inference (NLI) models to inference heuristics, as measured by the HANS evaluation set~\cite{mccoy2019right}. 
% \textbf{2) Minimizing human efforts in contrast set construction}
3) improving compositionality in \textbf{fine-grained style transfer} (\sect{sec:style_transfer}): \sysname achieves impressive zero-shot performance on fine-grained and compositional transfers in the \textsc{StylePTB} benchmark \citep{Lyu2021StylePTBAC}, even outperforming models trained on the dataset.

% We show that \sysname can help mitigate the data sparsity issues in various downstream tasks.
% In Natural Language Inference (NLI), we replicate perturbation strategies presented in HANS~\cite{mccoy2019right}, and use them to perturb the actual SNLI~\cite{bowman2015large} instances (instead of the templated data in HANS).
% The produced data, when automatically labeled, significantly improves NLI model generalization, on both HANS and other NLI challenge sets.
% In addition, \sysname helps replicate exisiting challenge sets on four diverse tasks, with much less manual annotation effort.
% We opensource \sysname at \opensourceurl.


==> sections/app_style_transfer.tex <==
\input{tables/stylePTB_results}

\section{Application 3: Style Transfer}
\label{sec:style_transfer}

Here, we show how \sysname can be applied to style transfer. 
We 
%formulate style transfer as a perturbation-based task and 
evaluate \sysname without any finetuning\footnote{This evaluation is zero-shot in spirit, as \sysname is not trained on any paired transfers present in \styleptb. 
%However, Ontonotes 5.0 does contain some overlap with the PTB \citep{van-son-etal-2018-resource}. 
However, it is unclear if the test inputs in \styleptb overlap with the Ontonotes 5.0 training data, since the two do share some data points~\citep{van-son-etal-2018-resource}, and \styleptb does not seem to preserve original PTB splits.
This leakage may advantage the external SRL predictor in parsing \styleptb test inputs. 
Still, this advantage should be minor, as the evaluated transfers do not require complex semantic role parsing.} on the \textsc{StylePTB} benchmark \citep{Lyu2021StylePTBAC}, which builds on the Penn Treebank and assesses fine-grained stylistic changes, both on \textit{single} transfers (\eg \textit{To Future Tense}) and compositional ones that concurrently edit multiple stylistic dimensions (\eg \textit{To Future Tense+ Active To Passive}).
%and assesses fine-grained stylistic changes (lexical, syntactic, semantic, and thematic), as well as compositions of multiple transfers. \textit{Single} transfers require editing an input sentence along one fine-grained stylistic dimension (\eg \textit{To Future Tense}). \textit{Compositional} transfers require editing along multiple stylistic dimensions at the same time (\eg \textit{To Future Tense+ Active To Passive}).

We evaluate \sysname on transfers for which \citet{Lyu2021StylePTBAC} show model results in the paper, excluding some that our semantic-role-derived inputs are not well-suited (see \sect{sec:appendix-style-transfer}). 
For each transfer, we create perturbations for each predicate in the original input, and report mean BLEU scores.\footnote{We report \texttt{Bleu\_1} from \texttt{nlg-eval} \citep{sharma2017nlgeval}.}
%using the procedure described in \sect{sec:perturbations}. 
Because this process results in multiple perturbations (one per verb), we choose the one with the lowest perplexity from \gptbaseline to represent the transfer. Unsuccessful transfers, either due to a failure of perturbation strategy (\eg no verbs are found by our SRL predictor) or due to a degenerate output (see \sect{sec:degenerations}), are given a BLEU score of 0.0. 
%\matt{reference to degenerate output again---this should go to details in an appendix, not a quick note in the conclusion}
% \footnote{We also show results on the test subset that filters out these bad generations (shown in Table \ref{tab:styleptb} as \textit{Filtered Test}).}

%\footnote{For instance, a \textit{To Future} perturbation could change the verb ``plan'' or ``announce'' in ``the agency plans to announce specific relief procedures in the coming days.''} 

We work with baselines reported by \citet{Lyu2021StylePTBAC}: \textbf{{\gptbaseline}} and \textbf{{\retrieveedit}} are the best-performing single-transfer models evaluated but require separate models to be trained for each transfer.
\textbf{{\csgpt}*} are models trained on compositional subsets of data (\eg \emph{Tense+Voice}, detailed in Table~\ref{tab:styleptb} caption). \textbf{\csgptzero} are ablations of {\csgpt}* trained only on corresponding individual changes but evaluated on compositional transfers.\footnote{\csgptzero refers to \textsc{CS-GPT-Zero} in \citet{Lyu2021StylePTBAC}.}

%\paragraph{Result.}
We report a subset of the comparisons in Table~\ref{tab:styleptb} (b), and the full result in Appendix~\ref{sec:appendix-style-transfer}. 
On compositional transfers, we find that \sysname outperforms the baseline system trained without compositional fine-tuning, \csgptzero, on 8/9 compositions, and even outperforms {\csgpt}* --- models with compositional finetuning --- on 5 cases.
% \wts{double check number?}
It also achieves compatible or better results than \gptbaseline and \retrieveedit on single transfers.
%outperforming 5/7 of the \gptbaseline and 1 of the \retrieveedit models finetuned on individual transfers. 
Low \sysname performance on some transfers
% have low performance 
(\eg \textit{ToFuture+ActiveToPassive}) appears to be driven by unsuccessful transfers, rather than generations that do not follow controls, as indicated by the higher performances on the subset where unsuccessful transfers are removed (\emph{Filtered Test}). 
Importantly, \sysname achieves these gains with a \emph{single model} and \emph{without any transfer-specific finetuning}.

==> sections/longer_discussion.tex <==
\section{Conclusion and Future Work}
\label{sec:discussion}

We propose \sysname, a flexible system that enables complex and context-aware perturbations useful for various downstream applications, including contrast set generation, data augmentation, and fine-grained style transfer.
\sysname demonstrates that it is possible to drive fine-grained perturbations with semantic features directly derived from an instance.
Crucially, it also shows that language models can be finetuned to learn representations of control codes, if paired with unlikelihood training, which encourages reliance on structured controls, rather than surrounding natural text.

\paragraph{Extending \sysname.} 
Besides the perturbation oriented tasks we explored, \sysname generator is well-suited for controlled generation tasks more broadly. 
Given key entities or arguments as keywords and fully masked contexts, we envision \sysname can help generate arguments~\cite{schiller2020aspect}, compositional data augmentation~\cite{akyurek2020learning}, caption generation~\cite{chen2020say}, etc.

The design of controls is also worthy of in-depth exploration.
As mentioned in \S\ref{sec:related}, AMR might be an alternative for semantic representation, if our primary goal is to 
%specify key entities and/or to 
express non-sequential relations.
On the other hand, dependency parsing labels are useful for syntactic changes; future work may try to balance syntactic and semantic controls.

\paragraph{Factors that affect \sysname's capability.} 
Though broadly applicable, \sysname's controllability and effectiveness varies with different inputs.
First, creating automatic perturbations with \sysname requires external SRL predictors, which can be noisy on some rare semantic roles.
% can add this back
%--- the one we use predicts core arguments more accurately than adjunct arguments (\eg F1 for \optag{ARG0} and \optag{ARGM-EXT} is 92.9 versus 51.4).
Empirically, most applications tend to modify common arguments, making the predictor applicable.
However, perturbing more challenging linguistic phenomena may require careful SRL predictor augmentation, or even manual semantic role annotation.

We also notice \sysname can produce degenerate outputs in some cases.
This may be a byproduct of unlikelihood training --- that the generator learns to reduce the likelihood of negative sequences by generating tokens that are very unlikely to appear in natural text. 
Certain generation hyperparameters, particularly the number of beams, can reduce the number of degenerate outputs.
While we perform unlikelihood training at the sequence level, future work can investigate the effect of penalizing generation at the level of tokens or spans, which may provide finer-grained signals for which spans should be considered unlikely, as well as more strategically balancing positive and negative samples. 

Having noted these opportunities, we believe \sysname is already a powerful tool for perturbation, particularly for tasks where compositional changes are required. 
\sysname is opensource, and available at \repourl.



==> sections/longer_related.tex <==
\section{Related Work}
\label{sec:related}

\paragraph{Controlled generation.}
Controllable text generation has been widely used to influence the various properties of generated text, for tasks like text summarization~\cite{peng2019text}, data augmentation~\cite{Lee2021NeuralDA}
style transfer~\cite{reid2021lewis, madaan2020politeness}, 
adversarial example generation~\cite{iyyer2018adversarial}, etc.
Most generators take simple attributes like 
tense~\cite{hu2017toward},
topic~\cite{Keskar2019CTRLAC}, and
sentiment polarity~\cite{Dathathri2020PlugAP}, which usually under specify the desired patterns.
In contrast, \sysname facilitates a variety of linguistically-driven generations, %using semantic roles and keywords, 
and therefore concretizes otherwise sparse controls. 
%(\eg we can specify making a sentence more negative \emph{through negation}.)
Recent work has explored using syntactic signals for paraphrasing~\cite{iyyer2018adversarial, kumar2020syntax}, which are similar to ours in their high-dimensional specification.
Still, to the best of our knowledge, \sysname is the first to incorporate fine-grained semantic controls.

Our generator is also related to methods for structured generation, which reconstruct sentences based on semantic representations.
Abstract Meaning Representation (AMR)~\cite{banarescu2013abstract, mager2020gpt} is an alternative representation worth exploring.
It presents the trade-off between training complexity and control flexibility: 
AMR may further enable controls on entity recursions~\citep{damonte2019structural}, but expressing such relationships in the inputs would be nontrivial.
However, when we omit these relationships and reduce AMR graphs to sequences (\eg like in~\cite{damonte2019structural}), semantic parses derived from PropBank have the advantage of enabling stricter control on \optag{complete} keywords, as they annotate complete spans, whereas AMR only accepts key entities without the syntactic sugar (\eg ``as,'' ``in'')~\cite{banarescu2013abstract}.

\paragraph{Data perturbation.}
Controlled generators have been shown to be particularly useful for text perturbation.
Besides the aforementioned paraphrasing and style transfer, prior works have also successfully generated contrastive examples that are useful for model training, evaluation, and explanation.
They usually rely on application-specific class labels~\cite{ross2020explaining, madaan2020generate, sha2021controllingtextedition, akyurek2020learning} or heuristic perturbation strategies that need to be expressed through pairs of original and perturbed sentences~\cite{polyjuice:acl21}, which are expensive to generalize. 
Recently, \citet{huang2021generating} designed SynPG, a paraphraser that can mimic parse tree structures learned from non-paired sentences.
We similarly train linguistically controlled generators on single sentences, but with a focus on fine-grained semantic perturbations which can be composed into broader types of changes.
%, such that we can more broadly cover different perturbation strategies by composing changes to control codes.

Also related are prior works creating minimally edited datasets through extensive human efforts -- either by manually rewriting instances~\cite{gardner2020evaluating, kaushik2019learning}, or by defining perturbation functions and templates (\eg~\cite{andreas-2020-good, li-etal-2020-linguistically, Ribeiro2020BeyondAB, wu-etal-2019-errudite}).
%Ribeiro2018SemanticallyEA, zhang-etal-2019-paws, kim2020cogs,
\S\ref{sec:contrast_set} shows that \sysname can help recreate many such datasets with less manual effort.
Moreover, the low overlap between \sysname's perturbations and humans' motivates future explorations of collaborative generation, where the generator can compensate humans' systematic omissions.

==> tables/OLD_hans_results.tex <==

\setlength{\tabcolsep}{5pt}

\begin{table}
\centering
\small
\renewcommand{\arraystretch}{0.9}
%\fontsize{8.5}{9.5}\selectfont

\begin{tabular}{@{} l|c|ccc @{}}
\toprule

& & \multicolumn{3}{c}{\textbf{HANS Subset}}\\
\textbf{Training Data} & \small \textbf{SNLI} &  \small \textbf{All} & \small \textbf{Entail.} & \textbf{Non-Entail.}\\


\midrule\midrule
SNLI Train 
& \textbf{91.12} %(0.21) 
& 64.72 %(1.85) 
& \textbf{98.95} %(0.47) 
& 30.46 %(3.99) 
\\
+ \sysname Perturb. 
& \textbf{91.12} %(0.19) 
& \textbf{66.45} %(1.49) 
& 97.97 %(1.41) 
& \textbf{34.92} \\ %(3.78)\\

\bottomrule
\end{tabular}
\vspace{-5pt}
\caption{
%We compare classifiers trained on just the SNLI train data vs. augmented with \sysname perturbations. 
% Compared to classifiers trained on just the SNLI train data, the 
\sysname augmentations lead to statistically significant gains on the HANS challenge set, without decreasing in-domain accuracy.}
%(averaged across 20 random seeds).
\vspace{-15pt}
\label{tab:hans-results}
\end{table}













==> tables/hans_perturbation_strategies.tex <==
\newcommand{\titlerule}{\arrayrulecolor{black!50}\midrule}
\renewcommand{\perturbname}[2]{\multicolumn{2}{p{\tablefrac\linewidth}}{\textbf{#1}: {#2}}}
\renewcommand{\subrule}{\arrayrulecolor{white!30}\midrule}
\renewcommand{\mainrule}{\arrayrulecolor{black!100}\midrule}


\begin{table*}
\centering
\footnotesize
\setlength{\tabcolsep}{5pt}

\begin{tabular}{@{} r | p{0.9\linewidth} @{}}
\toprule
%\multirow{20}{*}{\rotatebox[origin=c]{90}{\textbf{Meaning Preserving Strateges}}}

\multicolumn{2}{p{\tablefrac\linewidth}}{\textbf{Meaning Preserving Strategies}}\\
\midrule\midrule
\perturbname{Untangle relative clause} {For verbs with args containing relative clauses (\ie roles with \textit{R-}), delete context.}\\
\titlerule
Original & 
    The \tgenerate{PATIENT}{athlete} who was \tgenerate{VERB}{seen} \tgenerate{AGENT}{by the judges} \tgenerate{TEMPORAL}{yesterday} called the manager\\
\subrule 
Edits & 
    \optag{CONTEXT(DELETE\_TEXT)}\newline
    $\rightarrow$ [\theaderVerb{passive}{past}{see} | 
    \theader{AGENT}{complete}{by the judges} | \theader{PATIENT}{complete}{the athlete} | \theader{TEMPORAL}{complete}{yesterday}] 
    \tblank{0} \removesout{who} \tblank{1} \tblank{2} \tblank{3} \tblank{4} \removesout{called the manager}\\
\subrule
Perturb. & 
     The \tgenerate{PATIENT}{athlete} was \tgenerate{VERB}{seen} \tgenerate{AGENT}{by the judges} \tgenerate{TEMPORAL}{yesterday} \\
\mainrule


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\perturbname{Shorten core} {Change keywords for core args to root of original arg spans.}\\
\titlerule
Original & 
    The \tgenerate{AGENT}{athlete who was seen by the judges yesterday} \tgenerate{VERB}{called} \tgenerate{PATIENT}{the manager}.\\
\subrule 
Edits & 
    \optag{AGENT:CHANGE\_CONTENT(The athlete \removesout{who was...})}\newline
    $\rightarrow$ [\theaderVerb{active}{past}{call} | 
    \theader{AGENT}{complete}{The athlete \removesout{who was seen by the judges yesterday}} | \theader{PATIENT}{complete}{the manager}] 
    \tblank{0} \tblank{1} \tblank{2} \tblank{3} \tblank{4}\\
\subrule
Perturb. & 
     The \tgenerate{AGENT}{athlete} \tgenerate{VERB}{called} \tgenerate{PATIENT}{the manager}. \\
\mainrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\perturbname{Change voice}{Swap active/passive verb controls.}\\
\titlerule
Original & 
    The \tgenerate{AGENT}{athlete who was seen by the judges yesterday} \tgenerate{VERB}{called} \tgenerate{PATIENT}{the manager}.\\
\subrule 
Edits & 
    \optag{VERB:CHANGE\_VOICE(passive)|AGENT:CHANGE\_CONTENT(\add{by} the athlete who was...)}\newline
    $\rightarrow$ [\theaderVerb{\swap{active}{passive}}{past}{call} | 
    \theader{AGENT}{complete}{\add{by} the athlete who was seen by the judges yesterday} | \theader{PATIENT}{complete}{the manager}] 
    \tblank{0} \tblank{1} \tblank{2} \tblank{3} \tblank{4}\\
\subrule
Perturb. & \ \tgenerate{PATIENT}{The manager} was \tgenerate{VERB}{called} \tgenerate{AGENT}{by the athlete who was seen by the judges yesterday}. \\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\arrayrulecolor{black!100}\specialrule{.8pt}{2pt}{20pt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\arrayrulecolor{black!100}\toprule

\multicolumn{2}{p{\tablefrac\linewidth}}{\textbf{Meaning Changing Strategies}}\\
\midrule\midrule

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\perturbname{Replace core with subsequences}{Change keywords of core args to noun chunks from other args.}\\
\titlerule
    Original & 
    \ \tgenerate{AGENT}{The judge behind the manager} \tgenerate{VERB}{saw} \tgenerate{PATIENT}{the doctors}.\\
\subrule 
Edits & 
    [\theaderVerb{\swap{active}{passive}}{past}{call} | 
    \theader{AGENT}{complete}{\add{by} the athlete who was seen by the judges yesterday} | \theader{PATIENT}{complete}{the manager}] 
    \tblank{0} \tblank{1} \tblank{2} \tblank{3} \tblank{4}\\
\subrule
Perturb. & 
   \ \tgenerate{AGENT}{The doctors} \tgenerate{VERB}{saw} \tgenerate{PATIENT}{the manager}.\\
\mainrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\perturbname{Swap core}{Swap agent/patient.}\\
\titlerule
Original & 
   \ \tgenerate{PATIENT}{The athlete} who was \tgenerate{VERB}{seen} \tgenerate{AGENT}{by the judges} called the manager.\\
\subrule 
Edits & 
    \optag{SWAP\_CORE} \newline
    $\rightarrow$ [\theaderVerb{{passive}}{past}{see} | 
    \theader{AGENT}{complete}{by the \swap{judges}{athlete}} | \theader{PATIENT}{complete}{by the \swap{athlete}{judges}}] 
    \tblank{0} \tblank{1} \tblank{2} \tblank{3} \tblank{4}\\
\subrule
Perturb. & 
   \ \tgenerate{PATIENT}{The {judges}} who {were} \tgenerate{VERB}{seen} \tgenerate{AGENT}{by the {athlete}} called the manager.\\
\arrayrulecolor{black!100}\bottomrule

\end{tabular}
\caption{Overview of perturbation strategies we apply to SNLI hypotheses in our augmentation experiments (\sect{sec:data_augment}).}
\vspace{-15pt}
\label{tab:hans-strategies}
\end{table*}

==> tables/hans_perturbation_strategies_backup.tex <==
\newcolumntype{M}[1]{>{\arraybackslash}m{#1}}

\begin{table*}
\centering
\footnotesize
\setlength{\tabcolsep}{5pt}

\begin{tabular}{@{} M{0.18\linewidth}|M{0.82\linewidth} @{}}
\toprule
\multicolumn{2}{c}{\textbf{Meaning Preserving Strateges}} \\\midrule\midrule


\textbf{Untangle relative clause:} For verbs with args containing relative clauses (\ie SRL tags beginning \textit{B-R-}), delete context.
& 
\textbf{Original:} The \tgenerate{PATIENT}{athlete} who was \tgenerate{VERB}{seen} \tgenerate{AGENT}{by the judges} \tgenerate{TEMPORAL}{yesterday} called the manager

\textbf{Perturbed:} The \tgenerate{PATIENT}{athlete} was \tgenerate{VERB}{seen} \tgenerate{AGENT}{by the judges} \tgenerate{TEMPORAL}{yesterday} 
\newline

\optag{CONTEXT(DELETE\_TEXT)} $\rightarrow$ [\theaderVerb{passive}{past}{see} | 
    \theader{AGENT}{complete}{by the judges} | \theader{PATIENT}{complete}{the athlete} | \theader{TEMPORAL}{complete}{yesterday}] 
    \tblank{0} \removesout{who} \tblank{1} \tblank{2} \tblank{3} \tblank{4} \removesout{called the manager}
\\\midrule

%%%%%

\textbf{Shorten core:} Change keywords for core args to root of original arg spans.
& 
\textbf{Original:} The \tgenerate{AGENT}{athlete who was seen by the judges yesterday} \tgenerate{VERB}{called} \tgenerate{PATIENT}{the manager}.

\textbf{Perturbed:} The \tgenerate{AGENT}{athlete} \tgenerate{VERB}{called} \tgenerate{PATIENT}{the manager}.
\newline

\optag{AGENT:CHANGE\_CONTENT(The athlete \removesout{who was...})} $\rightarrow$ [\theaderVerb{active}{past}{call} | 
    \theader{AGENT}{complete}{The athlete \removesout{who was seen by the judges yesterday}} | \theader{PATIENT}{complete}{the manager}] 
    \tblank{0} \tblank{1} \tblank{2} \tblank{3} \tblank{4}
\\\midrule

%%%%%

\textbf{Change voice:} Swap active/passive verb controls.
& 
\textbf{Original:} The \tgenerate{AGENT}{athlete who was seen by the judges yesterday} \tgenerate{VERB}{called} \tgenerate{PATIENT}{the manager}.

\textbf{Perturbed:} \tgenerate{PATIENT}{The manager} was \tgenerate{VERB}{called} \tgenerate{AGENT}{by the athlete who was seen by the judges yesterday}.
\newline

\optag{VERB:CHANGE\_VOICE(passive)|AGENT:CHANGE\_CONTENT(\add{by} the athlete who was...)} \newline
$\rightarrow$ [\theaderVerb{\swap{active}{passive}}{past}{call} | 
    \theader{AGENT}{complete}{\add{by} the athlete who was seen by the judges yesterday} | \theader{PATIENT}{complete}{the manager}] 
    \tblank{0} \tblank{1} \tblank{2} \tblank{3} \tblank{4}
\\\midrule\midrule

\multicolumn{2}{c}{\textbf{Meaning Changing Strateges}} \\\midrule\midrule

%%%%%%%%%%
\textbf{Replace core with subsequences:} Change keywords of core args to noun chunks from other args.
&
\textbf{Original:} \tgenerate{AGENT}{The judge behind the manager} \tgenerate{VERB}{saw} \tgenerate{PATIENT}{the doctors}.

\textbf{Perturbed:} \tgenerate{AGENT}{The doctors} \tgenerate{VERB}{saw} \tgenerate{PATIENT}{the manager}.
\newline

\optag{AGENT:CHANGE\_CONTENT(The doctors)|PATIENT:CHANGE\_CONTENT(the manager)} \newline
$\rightarrow$ [\theaderVerb{\swap{active}{passive}}{past}{call} | 
    \theader{AGENT}{complete}{\add{by} the athlete who was seen by the judges yesterday} | \theader{PATIENT}{complete}{the manager}] 
    \tblank{0} \tblank{1} \tblank{2} \tblank{3} \tblank{4}
\\\midrule

%%%%%%%%%%
\textbf{Swap core:} Swap agent/patient.
&
\textbf{Original:} \tgenerate{PATIENT}{The athlete} who was \tgenerate{VERB}{seen} \tgenerate{AGENT}{by the judges} called the manager.

\textbf{Perturbed:} \tgenerate{PATIENT}{The {judges}} who {were} \tgenerate{VERB}{seen} \tgenerate{AGENT}{by the {athlete}} called the manager.
\newline

\optag{SWAP\_CORE} $\rightarrow$ [\theaderVerb{{passive}}{past}{see} | 
    \theader{AGENT}{complete}{by the \swap{judges}{athlete}} | \theader{PATIENT}{complete}{by the \swap{athlete}{judges}}] 
    \tblank{0} \tblank{1} \tblank{2} \tblank{3} \tblank{4}
\\


\bottomrule

\end{tabular}
\caption{Overview of perturbation strategies we apply to SNLI hypotheses in our augmentation experiments (\sect{sec:data_augment}).}
\vspace{-15pt}
\label{tab:hans-strategies}
\end{table*}

==> tables/intrinsic_ablation_backup.tex <==
\begin{table}[tb]
\small
    \centering
    \begin{tabular}{@{} l | r | r | r @{}}
    \toprule
    \multicolumn{4}{l}{\textbf{Closeness with the original sentence}}\\
    \midrule\midrule
    Models          & F1   & Precision       & Recall \\
      \midrule
    \textbf{\sysname}         & \textbf{64.3\%}   & \textbf{66.5\%}    & \textbf{73.4\%} \\
    \sysname$_{MLE}$ & 58.5\%   & 59.5\%    & 68.6\% \\
    \midrule\midrule

    \multicolumn{4}{l}{\textbf{Controllability on predicates}}\\
    \midrule\midrule
    Models          & Lemma   & Tense     & Voice \\
      \midrule
    \sysname         & \textbf{74.3\%}   & \textbf{80.3\%}    & \textbf{81.6\%} \\
    \sysname$_{MLE}$ & 72.2\%   & 70.2\%    & 76.1\% \\
    \midrule\midrule
    
    \multicolumn{4}{l}{\textbf{Controllability on arguments}}\\
    \midrule\midrule
    Models           & Role      & Content  & Specificity \\
      \midrule
    \sysname         & \textbf{70.5\%}    & \textbf{64.5\%}   & \textbf{64.5\%} \\
    \sysname$_{MLE}$ & 60.3\%    & 45.1\%   & 45.1\% \\
    
    \bottomrule
    \end{tabular}
    \vspace{-5pt}
    \caption{
    \sysname generates perturbations that are close to the original sentence, while reasonably following all the controls specified in Table~\ref{tab:controls}.
    Through an ablation study where unlikelihood training is removed (\sysname$_{MLE}$), we see that the controllability and closeness are both core benefits from unlikelihood training.}
    \vspace{-10pt}
    \label{table:intrinsic}
\end{table}

==> tables/perturbation_backup.tex <==
\begin{table*}[t!]
\centering
\small
\begin{tabular}{@{} p{0.25\linewidth} | p{0.65\linewidth} @{}}
\toprule
\textbf{\sysname Operations} & \textbf{Perturbed Part of Input/ Generated Text} \\
\midrule\midrule
	%%%%
	\multicolumn{2}{l}{\textbf{Syntactically controlled rewriting}}\\
	%%% 
	\midrule
	
	\multirow{2}{*}{\optag{CHANGE\_VTENSE(present)}} &
	{[\theaderVerb{active}{\swap{past}{present}}{comfort}]}\newline
	In the operation room, the doctor \add{comforts} the athlete.\\
	\midrule
	\multirow{2}{*}{\optag{CHANGE\_VVOICE(passive)}} &
	{[\theaderVerb{\swap{active}{passive}}{past}{comfort}]}\newline
	In the operation room, \add{the athlete was comforted by the doctor}.\\
	%%% 
	\midrule
	\multirow{2}{*}{\optag{CHANGE\_IDX(4:0)}} &
	{\add{\tblank{0}} In the operation room \remove{\tblank{0}}}\newline
	\add{{The doctor comforted the athlete}} in the operation room.
	\\
    \midrule
	%%%%
	\multirow{2}{*}{\optag{CORE(SWAP\_CORE)}} &
	{[\theader{AGENT}{complete}{the \swap{athlete}{doctor}}
| \theader{PATIENT}{complete}{the \swap{doctor}{athlete}} ]}\newline
	In the operation room, \add{the athlete} comforted \add{the doctor}.\\
\midrule\midrule
%%%%
\multicolumn{2}{l}{\textbf{Sentence expansion and abstraction}}\\
	\midrule
	%%% 
	\multirow{2}{\linewidth}{\optag{LOCATIVE:\newline CHANGE\_SPEC(partial)}} &
	{[\theader{LOCATIVE}{\swap{complete}{partial}}{in the operation room}]}\newline
	\add{Under the dim light} in the operation room, the doctor comforted the athlete.
% 	\\
	%%%%%
% 	\midrule
% 	\multirow{2}{\linewidth}{\optag{LOCATIVE:CHANGE\_CONTENT\newline(in the room)}} &
% 	{[\theader{LOCATIVE}{complete}{in the \removesout{operation} room}]}\newline
% 	In the \removesout{operation} room, the doctor comforted the athlete.
	\\
	%%%%%
	\midrule
	\multirow{2}{*}{\optag{LOCATIVE:DELETE}} &
	\removesout{{[\theader{LOCATIVE}{complete}{in the {operation} room}]}}\newline
	\removesout{In the operation room,} the doctor comforted the athlete.
	\\
	
\arrayrulecolor{black}\midrule\midrule
	%%%%
\multicolumn{2}{l}{\textbf{Data recombination (with external labels and/or contents)}}\\
	\midrule
	%%% 
% 	\multirow{2}{\linewidth}{\optag{AGENT:CHANGE\_CONTENT (the adult)}} &
% 	{[\theader{AGENT}{complete}{\swap{the doctor}{the adult}}]}\newline
% 	In the operation room the \add{adult} comforted the athlete.\\
% 	\midrule
	\multirow{4}{\linewidth}{\optag{CAUSE:CHANGE\_CONTENT\newline(because he was in pain)}} &
	Source sentence: \textit{The baby was crying because he was in pain.}\newline
	{[\theader{CAUSE}{complete}{\add{because he was in pain}}]}\newline
	In the operation room the doctor comforted the athlete \add{because he was in pain}.\\
\arrayrulecolor{black!100}\bottomrule
\end{tabular}
\vspace{-5pt}
\caption{We design a list of primitive operations on input controls to guide perturbations with the \sysname generator.}
\vspace{-10pt}
\label{table:optag}
\end{table*}



\newcommand{\subrule}{\arrayrulecolor{white!30}\midrule}
\newcommand{\mainrule}{\arrayrulecolor{black}\midrule}
\begin{table*}[h]
\fontsize{8}{9}\selectfont

\begin{subtable}[h]{ 0.45\textwidth}
\centering
\begin{tabular}{@{} p{0.14\textwidth} | p{0.87\textwidth} @{}}
\toprule
	%%%%
%\multicolumn{2}{l}{
& \textbf{Syntactically controlled rewriting}\\
	%%% 
\mainrule
	Strategy & 
	    \optag{CHANGE\_VTENSE(present)} \newline $\rightarrow$
	    [\theaderVerb{active}{\swap{past}{present}}{comfort}] \\
	\subrule
	Perturbed & 
	    In the operation room, the doctor \add{comforts} the athlete.\\

\mainrule
	Strategy &
	\optag{CHANGE\_VVOICE(passive)} \newline $\rightarrow$
	[\theaderVerb{\swap{active}{passive}}{past}{comfort}] \\
	\subrule
	Perturbed & 
	    In...room, \add{the athlete was comforted by the doctor}.\\
	%%% 
\mainrule
	Strategy & 
	    \optag{CHANGE\_IDX(4:0)} \newline $\rightarrow$
	    \add{\tblank{0}} In the operation room \remove{\tblank{0}}\\
	\subrule
	Perturbed & 
	    \add{{The doctor comforted the athlete}} in the operation room.\\
\mainrule
	%%%%
	Strategy & 
	    \optag{CORE(SWAP\_CORE)} \newline $\rightarrow$ [\theader{AGENT}{complete}{the \swap{athlete}{doctor}\newline
        | \theader{PATIENT}{complete}{the \swap{doctor}{athlete}} ]}\\
	\subrule
	Perturbed & 
	In the operation room, \add{the athlete} comforted \add{the doctor}.\\
\arrayrulecolor{black!100}\bottomrule
\end{tabular}
\end{subtable}


\hspace{10pt}

\begin{subtable}[h]{0.45\textwidth}
\centering
\begin{tabular}{@{} p{0.14\textwidth} | p{0.87\textwidth} @{}}
\toprule
%%%%
&\textbf{Sentence expansion and abstraction}\\
	\midrule
	%%% 
	\midrule
	Strategy & 
	    \optag{LOCATIVE:CHANGE\_SPEC(partial)} \newline $\rightarrow$
    	[\theader{LOCATIVE}{\swap{complete}{partial}}{in the operation room}]\\
	\subrule
	Perturbed & 
    	\add{Under the dim light} in the operation room, the doctor comforted the athlete.
% 	\\
	%%%%%
% 	\midrule
% 	\multirow{2}{\linewidth}{\optag{LOCATIVE:CHANGE\_CONTENT\newline(in the room)}} &
% 	{[\theader{LOCATIVE}{complete}{in the \removesout{operation} room}]}\newline
% 	In the \removesout{operation} room, the doctor comforted the athlete.
	\\
	%%%%%
	\midrule
	Strategy & 
	    \optag{LOCATIVE:DELETE} \newline $\rightarrow$
	    \removesout{{[\theader{LOCATIVE}{complete}{in the {operation} room}]}}\\
	\subrule
	Perturbed & 
	    \removesout{In the operation room,} the doctor comforted the athlete.
	\\
	
\arrayrulecolor{black}\midrule\midrule
	%%%%
\textbf{Data recombination (with external labels and/or contents)}\\
	\midrule
	%%% 
% 	\multirow{2}{\linewidth}{\optag{AGENT:CHANGE\_CONTENT (the adult)}} &
% 	{[\theader{AGENT}{complete}{\swap{the doctor}{the adult}}]}\newline
% 	In the operation room the \add{adult} comforted the athlete.\\
% 	\midrule
	{\optag{CAUSE:CHANGE\_CONTENT(because he was in pain)} \newline $\rightarrow$
	[\theader{CAUSE}{complete}{\add{because he was in pain}}]}\\
	\subrule
    	Perturbed & 
    	In the operation room the doctor comforted the athlete \add{because he was in pain}.\\
\arrayrulecolor{black!100}\bottomrule
\end{tabular}
\end{subtable}

\vspace{-5pt}
\caption{We design a list of primitive operations on input controls to guide perturbations with the \sysname generator.}
\vspace{-10pt}
\label{table:optag}
\end{table*}

==> tables/stylePTB_results.tex <==
\begin{table*}
\fontsize{8}{9}\selectfont
\centering

\renewcommand{\arraystretch}{0.85}

\begin{subtable}{1\textwidth}
\centering
\footnotesize
\setlength{\tabcolsep}{6.8pt}

\begin{tabular}{@{}p{0.22\textwidth} ||cc|cc| r r@{\hskip 3pt}r @{}}
\toprule

\multicolumn{1}{p{0.22\textwidth}||}{\multirow{4}{*}{(a) Single transfers}}

& \multicolumn{2}{c|}{\textbf{Single Finetune}} & \multicolumn{2}{c|}{\textbf{Compos. Finetune}} & \multicolumn{3}{c}{\textbf{No Finetune}}\\

\multicolumn{1}{l||}{} 
& \textbf{{\gptbaseline}*} & \textbf{{\retrieveedit}*} & 
\textbf{\csgpttv} & \textbf{\csgpttp} & \multicolumn{3}{c}{\textbf{\sysname}}\\

\cmidrule(lr){2-2}
\cmidrule(lr){3-3}
\cmidrule(lr){4-4}
\cmidrule(lr){5-5}
\cmidrule(lr){6-8}
\multicolumn{1}{l||}{} 
& Test & Test &Test & Test & Test & \multicolumn{2}{c}{Filtered Test} \\

\midrule\midrule
To Future Tense & 0.895 & \textbf{0.899} & 0.727 & 0.810 & 0.873 & 0.889 & (357/364)\\
%To Past Tense & 0.836 & \textbf{0.935} & 0.694 & 0.834 & 0.884 & 0.893 & (216/218)\\
%To Present Tense & 0.754 & \textbf{0.909} & 0.733 & 0.826 & 0.710 & 0.847 & (175/209)\\
ADJ or ADV Removal & 0.647 & \textbf{0.897} & --- & --- & 0.781 & 0.843 & (224/243)\\
PP Front to Back & 0.398 & 0.541 & --- & --- & \textbf{0.842} & 0.969 & (20/23)\\
%PP Removal & 0.763 & \textbf{0.798} & --- & 0.760 & 0.717 & 0.857 & (199/238) \\
Active to Passive & 0.476 & \textbf{0.681} & 0.472 & --- & 0.556 & 0.778 & (98/137)\\

\bottomrule
\end{tabular}
\label{tab:styleptb-single}
\end{subtable}



\vspace{0.2cm}


\setlength{\tabcolsep}{6.5pt}

\begin{subtable}{1\textwidth}
\footnotesize
\centering

\begin{tabular}{@{} ll||c|c| r r@{\hskip 3pt}r @{}}
\toprule

\multicolumn{2}{l ||}{\multirow{4}{*}{(b) Compositional transfers}}
& \multicolumn{1}{c|}{\textbf{Compos. Finetune}} & \multicolumn{1}{c|}{\textbf{Multi-Single Finetune}} & \multicolumn{3}{c}{\textbf{No Finetune}}\\

\multicolumn{1}{l}{} & \multicolumn{1}{c||}{} 
& \multicolumn{1}{c|}{\textbf{\csgpt}*}
& \multicolumn{1}{c|}{\textbf{\csgptzero}*} & \multicolumn{3}{c}{\textbf{\sysname}} \\

\cmidrule(lr){3-3}
\cmidrule(lr){4-4}
\cmidrule(lr){5-7}
\multicolumn{2}{l ||}{} & Test & Test & Test & \multicolumn{2}{c}{Filtered Test}  \\

\midrule\midrule

\multirow{4}{*}{\begin{tabular}{@{}l@{}}\textbf{Tense +} \\
\textbf{Voice}\end{tabular}} 
& ToPast+ActiveToPassive & 0.409 & 0.337 & \textbf{0.660} & 0.660 & $(30/30)$\\
& ToPast+PassiveToActive & 0.474 & 0.365 & \textbf{0.702} & 0.702  & $(65/65)$ \\
%& ToFuture+ActiveToPassive & \textbf{0.496} & 0.419 & 0.468 & 0.670 & ($90/131$)\\
%& ToFuture+PassiveToActive & 0.528 & 0.399 & \textbf{0.683} & 0.683  & $(131/131)$ \\
& ToPresent+ActiveToPassive & \textbf{0.503} & 0.445   & 0.315 & 0.614 & $(43/84)$\\
& ToPresent+PassiveToActive & 0.523 & 0.424 & \textbf{0.699} & 0.699 & $(95/95)$ \\
\midrule

\multirow{2}{*}{\begin{tabular}{@{}l@{}}\textbf{Tense +} \\
\textbf{PPRemoval}\end{tabular}} 
& ToPast+PPRemoval & \textbf{0.772} & 0.542 & 0.738 & 0.797 & $(100/108)$\\
& ToFuture+PPRemoval & 0.738 & 0.465 & \textbf{0.743} & 0.792 & $(215/229)$\\
%& ToPresent+PPRemoval & \textbf{0.709} & 0.545 & 0.691 & 0.704 & $(153/156)$\\

\bottomrule
\end{tabular}
\label{tab:styleptb-compositional}
\end{subtable}




\centering
\vspace{-5pt}
\caption{
BLEU scores for a subset of single and compositional style transfers in \styleptb (more in \S\ref{sec:appendix-style-transfer}).
Baseline results are taken from Tables 14-16 and 19-20 in \citet{Lyu2021StylePTBAC}.
%Best test results for each transfer (row) are bolded. 
%We also show results on \textit{Filtered Test}, which excludes \sysname degenerate outputs. 
* represents the same type of models finetuned on different subsets of styles, \eg {\csgpt}* in (b) includes \csgpttv, trained on all \textit{Tense+Voice} compositional transfers, and \csgpttp, on \textit{Tenses+PP Removal}.
A single \sysname model helps achieve comparable performance on single transfers compared to finetuned baselines, and is more capable on multiple compositional transfers. 
}
\label{tab:styleptb}
\vspace{-10pt}
\end{table*}




==> tables/unlikelihood_perturbations.tex <==
\begin{table*}
\centering
\small
\setlength{\tabcolsep}{5pt}

\begin{tabular}{@{} p{0.15\linewidth}|p{0.8\linewidth} @{}}
\toprule
\textbf{Description} & \textbf{Perturbation Strategy}\\
\midrule\midrule

\multirow{1}{*}{Change tags} & \multirow{1}{*}{\textcolor{cop}{\optag{VERB(CHANGE\_TENSE,CHANGE\_VOICE)}\optag{CORE(SWAP\_CORE)}\optag{NONCORE(ALL:CHANGE\_TAG)}}} \\\midrule

\multirow{1}{*}{Change keywords} & \multirow{1}{*}{\textcolor{cop}{\optag{VERB(CHANGE\_LEMMA)}\optag{CORE(ALL:CHANGE\_CONTENT)}\optag{NONCORE(ALL:CHANGE\_CONTENT)}}} \\\midrule

\multirow{1}{*}{Change specificities} & \multirow{1}{*}{\textcolor{cop}{\optag{CORE(ALL:CHANGE\_SPECIFICITY))}}} \\


\bottomrule

\end{tabular}
\caption{Perturbation strategies for generating unlikelihood examples.}
\vspace{-15pt}
\label{tab:unlikelihood-perturbations}
\end{table*}
